Disjunctive cuts in Mixed-Integer Conic Optimization

This paper studies disjunctive cutting planes in Mixed-Integer Conic Programming. Building on conic duality, we formulate a cut-generating conic program for separating disjunctive cuts, and investigate the impact of the normalization condition on its resolution. In particular, we show that a careful selection of normalization guarantees its solvability and conic strong duality. Then, we highlight the shortcomings of separating conic-infeasible points in an outer-approximation context, and propose conic extensions to the classical lifting and monoidal strengthening procedures. Finally, we assess the computational behavior of various normalization conditions in terms of gap closed, computing time and cut sparsity. In the process, we show that our approach is competitive with the internal lift-and-project cuts of a state-of-the-art solver.

==> tex/analysis.tex <==
\section{Linear relaxations are enough, revisited}
\label{sec:analysis}

    \todo[inline]{I think this section was more confusing than other. In addition, this result is not that useful in practice}

    We now study valid inequalities for disjunctive conic sets, starting with an extension of Proposition 1.4.3 in \cite{Ben-Tal2001} to disjunctive sets.
    \begin{lemma}
        \label{lemma:disjunctive_inequalities}
        Let $\D {=} \bigvee_{h=1}^{H} 
            \left\{
                A_{h} x {\Kgeq{\K_{h}}} b_{h}
            \right\}
        $
        with each $\D_{h} {=} \{ A_{h}x \Kgeq{\K_{h}} b_{h} \}$ well-posed.
        Then
        $ 
            \polar{\D}
            = \bigwedge_{h=1}^{H} \left\{
                \alpha = A_{h}^{T}u_{h}, \beta \leq b_{h}^{T}u_{h}, u_{h} \in \K_{h}^{*}
            \right\}.
        $
    \end{lemma}
    \begin{proof}
        Follows from $ \polar{\D} = \bigcap_{h=1}^{H} \polar{\D_{h}}$ and each $\D_{h}$ being well-posed.\qed
    \end{proof}

    Lemma \ref{lemma:disjunctive_inequalities} allows to give a constructive proof to Theorem \ref{thm:valid_inequalities_MICP}, which was initially stated in \cite{Bonami2012a}, though only with an existence proof.
    
    \begin{theorem}[Adapted from Theorem 3 of \cite{Bonami2012a}]
        \label{thm:valid_inequalities_MICP}
        Let $P$ be given by \eqref{eq:MICP} and $L \leq U \in \R$ such that $\C \subseteq [L, U]^n$. Assume that, for every $h \in \Z^{p} \cap [L, U]^{p}$, $\{ Ax \Kgeq{\K} b, B_{h}x \geq d_{h} \}$ is well-posed, where $B_{h}x \geq d_{h}$ encodes $\{ x_{j} {=} h_{j}, j{=}1,...,p \}$.\\
        Then, if $(\alpha, \beta) \in \polar{\X}$, there exists $\tilde{A}$ and $\tilde{b}$ such that $\C \subseteq \{ \tilde{A} x \geq \tilde{b} \}$ and $(\alpha, \beta) \in \polar{\tilde{\X}}$, where $\tilde{\X} = \{x \in \Z^{p} \times \R^{n-p} | \tilde{A}x \geq \tilde{b} \}$.
    \end{theorem}
    \begin{proof}
        Let $\mathcal{H} = \Z^{p} \cap [L, U]^{p}$ and, for $h \in \mathcal{H}$, define $\D_{h} = \{ Ax \Kgeq{\K} b, B_{h}x \geq d_{h} \}$.
        Then, let $\D = \bigvee_{h} \D_{h}$ and note that, by construction, we have $\X = \D$.
        
        Let $(\alpha, \beta) \in \polar{\X} = \polar{\D}$.
        Thus, by Lemma \ref{lemma:disjunctive_inequalities}, there exists $u_{h} \in \K^{*}, v_{h} \geq 0$ such that $\alpha = A^{T}u_{h} + B_{h}^{T}v_{h}$ and $\beta \leq b^{T}u_{h} + d_{h}^{T}v_{h}, \forall h \in \mathcal{H}$.
        Then, consider
        \begin{align*}
        	(\tilde{P}) \ \ \ 
        	\min_{x} \ \ \ & c^{T}x \\
        	s.t. \ \ \
        	& (u_{h}^{T}A) x \geq u_{h}^{T}b, \ \ \ \forall h \in \mathcal{H},\\
        	& L \leq x_{j} \leq U, \ \ \ \ \ \ \ \forall j \in \{1, ..., n\},\\
        	& x \in \Z^{p} \times \R^{n-p},
        \end{align*}
        with feasible set $\tilde{\X}$.
        By construction, $\tilde{P}$ is an outer approximation of $P$.
        Then, define $\tilde{\D} = \bigvee_{h} \left\{(u_{h}^{T}A)x \geq u_{h}^{T}b, B_{h}x \geq d_{h} \right\}$.
        It is straightforward to verify that $(\alpha, \beta) \in \polar{\tilde{\D}} \subseteq \polar{\tilde{\X}}$, which concludes the proof.
        \qed
    \end{proof}
    
    Finally, note that the obtained outer-approximation in this proof is exponentially large.
    This is not a conservative estimate.
    Indeed, this can be the case if $\alpha = c$, since there exist  instances for which an outer-approximation algorithm requires exponentially many iterations to converge, see, e.g., Section 3 of \cite{Lubin2018}.
    
    
\iffalse
    Recall 
    \begin{align*}
    	(P) \ \ \ 
    	\min_{x} \ \ \ & c^{T}x \\
    	s.t. \ \ \
    	& Ax \Kgeq{\K} b,\\
    	& x \in \Z^{p} \times \R^{n-p},
    \end{align*}
    and assume that the feasible set $\X$ is bounded.
    Let $l_{i}, u_{i}$ be finite bounds such that $\forall x \in \X, l_{j} \leq x_{j} \leq u_{j}$.
    For simplicity, we assume $l = 0, u=1$, i.e., all integer variables are binaries.
    No loss of generality since we're considering a bounded set.
    
    Then, for every $h \in \{0, 1\}^{p}$, let $\D_{h} = \{Ax \Kgeq{\K} b, B_{h}x \geq d_{h} \}$ where $B_{h}x \geq d_{h}$ encodes $x_{j} = h_{j}, \forall j \in 1, ..., p$.
    We assume that every $\D_{h}$ is well-posed (it's essentially the same as Hypothesis 1 in \cite{Bonami2012}).
    Then let $\alpha, \beta$ be a valid inequality for $\X$.
    Since $\X = \D$, we have $u_{h} \in \K^{*}, v_{h}$ such that
    \begin{align}
        \forall h, \alpha &= A^{T}u_{h} + B_{h}^{T}v_{h}\\
        \forall h, \beta &\leq b^{T}u_{h} + d_{h}^{T}v_{h}
    \end{align}
    Then, consider the outer approximation
    \begin{align*}
    	(\tilde{P}) \ \ \ 
    	\min_{x} \ \ \ & c^{T}x \\
    	s.t. \ \ \
    	& (u_{h}^{T}A) x \geq u_{h}^{T}b, \ \ \ \forall h,\\
    	& 0 \leq x_{j} \leq 1, \forall j \in \{1, ..., p\}\\
    	& x \in \Z^{p} \times \R^{n-p},
    \end{align*}
    and the valid disjunction
    \begin{align}
        \tilde{\D} = \bigvee \left\{u_{h}^{T}Ax \geq u_{h}^{T}b, B_{h}x \geq d_{h} \right\}
    \end{align}
    Now, set $\lambda_{h} =1$, we have
    \begin{align}
        \forall h, \alpha &=  (A^{T}u_{h}) \lambda_{h} + B_{h}^{T}v_{h}\\
        \forall h, \beta &\leq (u_{h}^{T}b) \lambda_{h} + d_{h}^{T}v_{h}
    \end{align}
    thus $(\alpha, \beta) \in \polar{\tilde{\D}}$ and $\alpha, \beta$ is valid for $\tilde{\X}$.
\fi
    
\iffalse
    % Original wording of the proof
    Assume that the domain of the MICP is bounded, i.e., there are a finite number of possible integer assignments.
    Then, assume that all sub-problems are well-posed, i.e., they are either strongly feasible or strongly infeasible.
    Then consider the (finite) disjunction
    \begin{align*}
        \D &= \bigvee \left\{ Ax \Kgeq{\K} b, B_{i}x \geq d_{i} \right\}
    \end{align*}
    that contains one term for each feasible integer point.
    Thus $\D$ is exactly the feasible set of MICP, so that any valid inequality for $\D$ is valid for the MICP.
    
    Under the well-posed assumption, we can write
    \begin{align*}
        \alpha &= A^{T}u_{i} + B_{i}^{T}v_{i}\\
        \beta &\leq u_{i}b + v_{i}^{T}d_{i} \\
        u_{i} &\in \K^{*}
    \end{align*}
    
    and then consider the linear relaxation
    \begin{align}
        \tilde{C} &= \left\{
            x
        \ \middle| \  
            u_{i}^{T}A_{i}x \geq u_{i}^{T}b
        \right\}
    \end{align}
\fi
    
\iffalse
    {\blue
    The following lemma gives algebraic representations of valid inequalities for conic sets, and states sufficient conditions for this representation to be complete (i.e. all valid inequalities are represented).
    }
    
    For terminology, we shall refer to $u$ as a \emph{Farkas multiplier}, implying that $u$ is used to aggregate constraints into a valid inequality.
    
    {\blue
    Let us make the following remarks.
    \begin{enumerate}
        \item We have an algebraic description for the set of ``valid" Farkas multipliers: it is the dual cone $\Kb^{*}$.
        Note that this representation is compact and tractable.
        \item Whenever the system $\C$ is well-posed, we have a \emph{complete} representation of the set of valid inequalities
    \end{enumerate}
    }
    
    {\color{red}
    See Example 1.4.3 in \cite{Ben-Tal2001} for an example where a valid inequality cannot be obtained via Farkas aggregation.
    Consider the set 
    \begin{align}
        \C = \left\{
            (x_{1}, x_{2})
        \middle|
            \begin{pmatrix}
                x_{1}\\
                x_{2}\\
                x_{1}
            \end{pmatrix}
            \geq_{\mathcal{L}^{3}} 0
        \right\}.
    \end{align}
    It is trivial to see that $\C = \R_{+} \times \{0\}$ and that $x_{2} \geq 0$ is a valid inequality for $\C$.
    However, the system
    \begin{align}
        u_{1} + u_{3} &= 0,\\
        u_{2} &= 1,\\
        (u_{1}, u_{2}, u_{3}) &\in \mathcal{L}^{3},
    \end{align}
    has no solution.
    }
    
    
\subsection{Disjunctive inequalities}
\label{sec:notations:subsec:disjunctions}

    Consider a finite disjunction
    
    
    {\color{red}
        Unless specified otherwise, we assume that 
    }
    \todo[inline]{Note that facial reduction can be used to reduce an ill-posed problem into a well-posed one.}
    
    \begin{theorem}
        Let
        \begin{align}
            \D = \bigvee_{i=1}^{K} 
            \underbrace{
                \left\{
                    x
                \ \middle| \ 
                    A_{i} x \geq_{\K_{i}} b_{i}
                \right\}
            }_{\D_{i}}.
        \end{align}
        and assume that each individual disjunctive term $A_{i}x \geq b_{i}$ is well-posed.\\
        Then $(\alpha, \beta) \in  \polar{\D}$ if and only if there exists $u_{1}, ..., u_{K} \in \K_{1}^{*} \times ... \times \K_{K}^{*}$ such that
        \begin{align*}
            \forall i, \ \ \alpha &= A_{i}^{T}u_{i}, \ \ \beta \leq b_{i}^{T}u_{i}.
        \end{align*}
    \end{theorem}
    \begin{proof}
        Immediate from the fact that $ \polar{\D} = \bigcap_{i} \polar{\D_{i}}$ and each disjunctive term is well-posed.
    \end{proof}
    
    The example below shows how the above result fails miserably without the well-posed assumption.\\
    {\color{red}
        \textbf{[Problematic counter-example]}\\
        Consider the two-term disjunction
        \begin{align}
            \D = \left\{
                (x_{1}, x_{2})
            \ \middle | \ 
                \begin{pmatrix}
                    x_{1} \\ x_{2} \\ x_{1}
                \end{pmatrix}
                \geq_{\mathcal{L}^{3}}
                0
            \right\}
            \cup
            \left\{
                (x_{1}, x_{2})
            \ \middle | \ 
                \begin{pmatrix}
                    -x_{1} \\ x_{2} \\ x_{1}
                \end{pmatrix}
                \geq_{\mathcal{L}^{3}}
                0
            \right\}
        \end{align}
        One trivially verifies that $\D_{1} = \{x_{1} \geq 0, x_{2} = 0\}$ and $\D_{2} = \{x_{1} \leq 0, x_{2} = 0\}$, and it follows that $x_{2} \geq 0$ is a valid inequality for $\D$.
        
        However, the system
        \begin{align*}
            \alpha_{1} &= u_{1}+u_{3} = -v_{1} + v_{3}\\
            \alpha_{2} &= u_{2} = v_{2}\\
            \beta &\leq 0\\
            u, v &\in \mathcal{L}^{3}
        \end{align*}
        has no solution no matter the choice of $\alpha$.
        
        However, $x_{2} \geq 0$ is not representable by valid Farkas aggregation for neither $\D_{1}$ nor $\D_{2}$. In addition, any valid inequality for $D_{1}$ that is not parallel to $x_{2} = 0$ must cut the line $x_{2} = 0$ at a non-positive coordinate, and is therefore not valid for $\D_{2}$. Same by exchanging role.
    }
    
    
% \subsection{Linear relaxations}

%     Bonami \cite{Bonami2012b} gives an existence proof that any valid linear inequality can be obtained from a valid linear relaxation of the problem.
%     Here we give a constructive proof.
    
%     Assume that the domain of the MICP is bounded, i.e., there are a finite number of possible integer assignments.
%     Then, assume that all sub-problems are well-posed, i.e., they are either strongly feasible or strongly infeasible.
%     Then consider the (finite) disjunction
%     \begin{align*}
%         \D &= \bigvee \left\{ Ax \Kgeq{\K} b, B_{i}x \geq d_{i} \right\}
%     \end{align*}
%     that contains one term for each feasible integer point.
%     Thus $\D$ is exactly the feasible set of MICP, so that any valid inequality for $\D$ is valid for the MICP.
    
%     Under the well-posed assumption, we can write
%     \begin{align*}
%         \alpha &= A^{T}u_{i} + B_{i}^{T}v_{i}\\
%         \beta &\leq u_{i}b + v_{i}^{T}d_{i} \\
%         u_{i} &\in \K^{*}
%     \end{align*}
    
%     and then consider the linear relaxation
%     \begin{align}
%         \tilde{C} &= \left\{
%             x
%         \ \middle| \  
%             u_{i}^{T}A_{i}x \geq u_{i}^{T}b
%         \right\}
%     \end{align}
%     and the disjunction
%     \begin{align*}
        
%     \end{align*}
\fi
